An SDE perspective on stochastic convex optimization

We analyze the global and local behavior of gradient-like flows under stochastic errors towards the aim of solving convex optimization problems with noisy gradient input. We first study the unconstrained differentiable convex case, using a stochastic differential equation where the drift term is minus the gradient of the objective function and the diffusion term is either bounded or square-integrable. In this context, under Lipschitz continuity of the gradient, our first main result shows almost sure convergence of the objective and the trajectory process towards a minimizer of the objective function. We also provide a comprehensive complexity analysis by establishing several new pointwise and ergodic convergence rates in expectation for the convex, strongly convex, and (local) {\L}ojasiewicz case. The latter, which involves local analysis, is challenging and requires non-trivial arguments from measure theory. Then, we extend our study to the constrained case and more generally to certain nonsmooth situations. We show that several of our results have natural extensions obtained by replacing the gradient of the objective function by a cocoercive monotone operator. This makes it possible to obtain similar convergence results for optimization problems with an additively "smooth + non-smooth" convex structure. Finally, we consider another extension of our results to non-smooth optimization which is based on the Moreau envelope.

==> tex/sec-Conclusion.tex <==
\section{Conclusion, Perspectives}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This work was intended to uncover the global and local convergence properties of trajectories of gradient-like flows under stochastic errors. The aim is to solve convex optimization problems with noisy gradient input with vanishing variance. We have shed light on these properties and provided a comprehensive local and global complexity analysis both in the smooth and non-smooth case. We believe that this work paves the way to many important extensions and research avenues. Among them, we mention the following ones:

\smallskip

\begin{itemize}
\item Extension beyond the convex case, and for instance to the quasi-convex case.

\item Analyzing the case of a general maximal monotone operator which is merely Lipschitz continuous. This covers many important cases that are not covered by the analysis in this paper.

\item Understanding the behavior of the solution $X_{\theta}$ of \eqref{CSGD_theta} as $\theta$ vanishes is also a very interesting but challenging problem that we leave for future work.
\end{itemize}

==> tex/sec-Discrete.tex <==
\section{Discrete setting}\label{sec:discrete}

\begin{definition}
Consider $f:\R^d\rightarrow (-\infty,\infty]$, $f\in \Gamma_0(\R^d)$ and $\theta>0$, the Moreau envelope of $f$ of parameter $\theta$ is $$^{\theta}f(x)=\inf_{y\in\R^d} \left(f(y)+\frac{1}{2\theta}\Vert x-y\Vert^2\right)=\left(f \hspace{0.1cm}\square \hspace{0.1cm} \frac{q}{\theta}\right)(x),$$
where $q(x)=\frac{1}{2}\Vert x\Vert^2$.
\end{definition}
%Continuous Stochastic Results
\begin{proposition}\label{prim}
 Consider $f\in \Gamma_0(\R^d)$, then $^{\theta}f$ is convex, differentiable and has Lipschitz continuous gradient with constant $\frac{1}{\theta}$, in other words $^{\theta}f\in C_{\frac{1}{\theta}}^{1,1}(\R^d)\cap\Gamma_0(\R^d)$.
\end{proposition}
\begin{proposition}\label{sc}
 Consider $f\in \Gamma_c(\R^d)$, then $^{\theta} f$ is $\frac{c}{1+\theta c}-$strongly convex, in other words $^{\theta} f\in \Gamma_{\frac{c}{1+\theta c}}(\R^d) $.
\end{proposition}
\begin{proposition}\label{des}
 Consider $f\in \Gamma_0(\R^d)$, $\theta>0$, $^{\theta}f$ and $x\in \R^d$, then \begin{enumerate}[label=(\roman*)]
     \item $^{\theta}f(x) \downarrow inf f(\R^d)$ as $\theta\uparrow +\infty$.
     \item $^{\theta}f(x) \uparrow  f(x)$ as $\theta\downarrow 0$.
     \item $^{\theta}f(x)\leq f(x)$.
     \item $argmin(^{\theta}f)=argmin(f)$.
     \item If $D:=\sup_{x\in\R^d}\Vert\partial^0 f(x)\Vert<\infty$, then $f(x) -$ $^\theta f(x)\leq \theta D^2.$
 \end{enumerate}
\end{proposition}
\begin{proposition}\label{nuevo}
 Consider $f\in\Gamma_0(\R^d)$ such that $S:= argmin(f)\neq\varnothing$. Consider $\theta>0$, $^{\theta}f$ and suppose that $D:=\sup_{x\in\R^d}\Vert\partial^0 f(x)\Vert<\infty$. Let $X^{\theta}$ the solution of \eqref{CSGD} for the potential $^{\theta} f$. Then the following statements holds:
 \begin{enumerate}
     \item Since $f$ is convex, then $$\mathbb{E}(f(\overline{X^{\theta}}(t))-min(f))\leq \frac{d^2(X_0,S)}{2t}+\frac{\sigma_*^2 d}{2}+\theta D^2.$$
     \item If $f\in \Gamma_c(\R^d)$, consider $\mu=\frac{c}{1+\theta c}$, then $$\mathbb{E}\left(\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right)\leq \frac{d^2(X_0,S)}{2}e^{-\mu t}+\frac{\sigma_*^2 d}{2\mu}.$$
     \item If $f\in \Gamma_c(\R^d)$, consider $\mu=\frac{c}{1+\theta c}$, then
     $$\mathbb{E}(f(X^{\theta}(t))-min(f))\leq \frac{1}{\theta}\left(\frac{d^2(X_0,S)}{2}e^{-\mu t}+\frac{\sigma_*^2 d}{2\mu}\right)+\theta D^2$$
 \end{enumerate}
\end{proposition}
\begin{proof}
 \begin{enumerate}
     \item Direct from (i) of Theorem \ref{importante0}, (iv) and (v) of Proposition \ref{des}.
     \item Direct from (ii) of Theorem \ref{importante0} and Proposition \ref{sc}.
     \item Direct from (\ref{scr2}), (iv) and (v) of Proposition \ref{des}.
 \end{enumerate}
\end{proof}
\newpage
\begin{corollary}\label{nuevocor}
Under the same context as in Proposition \ref{nuevo}, consider $\varepsilon>0$. The following statement holds:
\begin{enumerate}
    \item Since $f$ is convex, if $ \theta=\mathcal{O}(min\{\sigma_*^2 d,\varepsilon\})$ and $t=\Omega\left(\frac{1}{\varepsilon}\right)$. Then $$\mathbb{E}[f(\overline{X^{\theta}}(t))-min(f)]=\mathcal{O}(max\{\sigma_*^2 d,\varepsilon\}).$$
    \item If $f\in \Gamma_c(\R^d)$ $(S=\{x^*\}), \theta=min\{\sigma_*^2 d,\varepsilon\}$ and $t=\Omega\left(ln \left(\frac{1}{\varepsilon}\right)\right)$. Then $$\mathbb{E}\left[\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right]=\mathcal{O}(max\{\sigma_*^2 d,\varepsilon\}).$$ 
    \item If $f\in \Gamma_c(\R^d), \theta=\mathcal{\sigma_*}$ and $t=\Omega\left(ln \left(\frac{1}{\sigma_*^2 d}\right)\right)$. Then $$\mathbb{E}[f(X^{\theta}(t))-min(f)]=\mathcal{O}(\sigma_*).$$
\end{enumerate}
\end{corollary}
\begin{proof}
 \begin{enumerate}
     \item Consider $t\geq \frac{d^2(X_0,S)}{2\varepsilon}, \theta=\frac{min\{\sigma_*^2 d,\varepsilon\}}{D^2}$. By Proposition \ref{nuevo}-1., we obtain that $$\mathbb{E}[f(\overline{X^{\theta}}(t))-min(f)]\leq \varepsilon+min\{\sigma_*^2 d,\varepsilon\}+\frac{\sigma_*^2 d}{2}=\mathcal{O}(\sigma_*^2 d+\varepsilon)=\mathcal{O}(max\{\sigma_*^2 d,\varepsilon\}).$$
     \item Consider $\theta=min\{\sigma_*^2 d,\varepsilon\}$. $t\geq \left(\frac{1}{c}+min\{\sigma_*^2 d,\varepsilon\}\right)ln\left(\frac{d^2(X_0,S)}{2\varepsilon}\right).$ By Proposition \ref{nuevo}-2., we obtain that $$\mathbb{E}\left[\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right]\leq \varepsilon+\frac{\sigma_*^2 d}{2c}+\sigma_*^3=\mathcal{O}(\sigma_*^2 d+\varepsilon)=\mathcal{O}(max\{\sigma_*^2 d,\varepsilon\}).$$
     \item Consider $\theta=\frac{\sigma_*}{D^2}, t\geq \left(\frac{1}{c}+\frac{\sigma_*}{D^2}\right)ln\left(\frac{d^2(X_0,S)}{2\sigma_*^2 d}\right)$. By Proposition \ref{nuevo}-3., we obtain that $$\mathbb{E}[f(X^{\theta}(t))-min(f)]\leq \left(2+\frac{1}{2c}\right)\sigma_*+\frac{\sigma_*^2 d}{2}=\mathcal{O}(\sigma_*).$$
 \end{enumerate}
\end{proof}

\begin{proposition}\label{pp}
 Consider $f,g$ such that $f$ is lower bounded and $g$ is convex and $L_0$-Lipschitz. Let $F:=f+g$, $\bar{\theta}>0$ and $F_{\theta}=f+$ $^{\theta}g$, where $\theta\in (0,\bar{\theta})$. Assuming that $argmin(F),argmin(^{\theta} F)\neq\varnothing$ and that $F$ is coercive, then there exists $C\geq 0$ such that $$\sup_{z\in argmin(F_{\theta})}\Vert z\Vert\leq C.$$  
\end{proposition}
\begin{proof}
 Let $x_{\theta}^*\in argmin(F_{\theta})$ and $x^*\in argmin(F)$ arbitrary. By Proposition \ref{des}, (v) we obtain $$F(x_{\theta}^*)\leq F_{\theta}(x_{\theta}^*)+L_0^2\theta.$$
 Moreover, $$F_{\theta}(x_{\theta}^*)+L_0^2\theta\leq F_{\theta}(x^*)+L_0^2\theta\leq F(x^*)+L_0^2\theta\leq min(F)+L_0^2\bar{\theta}=:\tilde{C}.$$
 Where the second inequality is given by (iv) of Proposition \ref{des}. On the other hand, the coercivity of $F$ implies that there exists $a>0,b\in\R$ such that $$a\Vert x\Vert+b\leq F(x).$$
Therefore, $$a\Vert x_{\theta}^*\Vert+b\leq F(x_{\theta}^*)\leq \tilde{C}.$$ Taking the supremum over $x_{\theta}^*$ and defining $C:=\frac{\tilde{C}-b}{a}\geq 0$, we obtain $$\sup_{z\in argmin(F_{\theta})}\Vert z\Vert<C.$$  
\end{proof}
\begin{corollary}
Let $X_0\in\R^d$, $\bar{\theta}>0$ and $\theta\in (0,\bar{\theta})$, then there exists $C\geq 0$ such that $$d(X_0,argmin(F_{\theta}))\leq \Vert X_0\Vert+C,$$
\end{corollary}
\begin{proof}
 Use the triangle inequality to go from $X_0$ to $argmin(F_{\theta})$ via $0$ and then Proposition \ref{pp}.
\end{proof}
\begin{proposition}\label{nuevo1}
 Consider $f\in\Gamma_0(\R^d)\cap C_\Lp^{1,1}(\R^d)$ and $g\in\Gamma_0(\R^d)$ such that is $L_0-$Lipschitz. Consider $\bar{\theta}>0$, $\theta\in (0,\bar{\theta})$ and let $X^{\theta}$ the solution of \eqref{CSGD} for the potential $f+$ $^{\theta} g$ and $S':= argmin(f+^{\theta}g)$ is nonempty. Then $d(X_0,S')\leq C_0$ and the following statement holds:
 \begin{enumerate}
     \item Since $f+g$ is convex, then $$\mathbb{E}((f+g)(\overline{X^{\theta}}(t))-min(f+g))\leq \frac{d^2(X_0,S')}{2t}+\frac{\sigma_*^2 d}{2}+\theta L_0^2.$$
     \item If $f\in \Gamma_{\mu'}$ ($S'=\{x^*\}$), then $$\mathbb{E}\left(\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right)\leq \frac{\Vert X_0-x^*\Vert^2}{2}e^{-\mu' t}+\frac{\sigma_*^2 d}{2\mu'}.$$
     \item If $f\in \Gamma_{\mu'}$, then $$\mathbb{E}((f+g)(X^{\theta}(t))-min(f+g))\leq \left(L+\frac{1}{\theta}\right)\left(\frac{\Vert X_0-x^*\Vert^2}{2}e^{-\mu' t}+\frac{\sigma_*^2 d}{2\mu'}\right)+\theta L_0^2.$$
     \item If $g\in \Gamma_c(\R^d)$ ($S'=\{x^*\}$), consider $\mu=\frac{c}{1+\theta c}$, then $$\mathbb{E}\left(\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right)\leq \frac{\Vert X_0-x^*\Vert^2}{2}e^{-\mu t}+\frac{\sigma_*^2 d}{2\mu}.$$
     \item If $g\in \Gamma_c(\R^d)$, consider $\mu=\frac{c}{1+\theta c}$, then
     $$\mathbb{E}((f+g)(X^{\theta}(t))-min(f+g))\leq \left(L+\frac{1}{\theta}\right)\left(\frac{\Vert X_0-x^*\Vert^2}{2}e^{-\mu t}+\frac{\sigma_*^2 d}{2\mu}\right)+\theta L_0^2.$$
     \item If $f\in \Gamma_{\mu'}$ and $g\in \Gamma_c(\R^d)$ ($S'=\{x^*\}$), consider $\mu=\frac{c}{1+\theta c}$. Then $$\mathbb{E}\left(\frac{\Vert X^{\theta}(t)-x^*\Vert^2}{2}\right)\leq \frac{\Vert X_0-x^*\Vert^2}{2}e^{-(\mu+\mu') t}+\frac{\sigma_*^2 d}{2(\mu+\mu')}.$$
     \item If $f\in \Gamma_{\mu'}$ and $g\in \Gamma_c(\R^d)$ ($S'=\{x^*\}$), consider $\mu=\frac{c}{1+\theta c}$. Then
     $$\mathbb{E}((f+g)(X^{\theta}(t))-min(f+g))\leq \left(L+\frac{1}{\theta}\right)\left(\frac{\Vert X_0-x^*\Vert^2}{2}e^{-(\mu+\mu') t}+\frac{\sigma_*^2 d}{2(\mu+\mu')}\right)+\theta L_0^2.$$
 \end{enumerate}
\end{proposition}
\begin{proof}
Direct from Proposition \ref{sc}, Proposition \ref{nuevo} and the fact that $$min(f+^{\theta} g)\leq min(f+g).$$
\end{proof}
%\begin{proof}
% \begin{enumerate}
%     \item Direct from (i) of Theorem \ref{importante0}, (iii) and (v) of Proposition \ref{nuevo}.
%     \item Direct from (ii) of Theorem \ref{importante0} and Proposition \ref{sc}.
%     \item Direct from (\ref{scr2}), (iii) and (v) of Proposition \ref{nuevo}.
% \end{enumerate}
%\end{proof}

   
     
     
% -se mostraron algoritmos y sus convergencias\\
 
% -vimos nuevos resultados para sgd discreto\\
 
% -vimos nuevos resultados para un modelo de sgd continuo inspirados en lo visto en \cite{optch}, \cite{mertikopoulos_staudigl_2018} and \cite{tailed}. \\ 
 
% -si asumiamos que $sigma_*^2$ es chiquito entonces obtenemos las complejidades esperadas\\
 
%  -poner tablas de complejidad con mas detalle i.e. decir que en sgd discreto loj se asumio $\bar{\sigma}^2<\infty$ o que en sgd discreto fuerte convexo no se uso stepsize fijo quizas\\
 
 %-como en sgd discreto no se asume eso toda esa tabla se ve diferente\\
 \begin{proposition}
 Let $\omega:\mathbb{R}^d\rightarrow\mathbb{R}$ a convex function such that $\omega\in C_{\frac{1}{\sigma}}^{1,1}(\mathbb{R}^d)$ for some $\sigma>0$ and let $g:\mathbb{R}^d\rightarrow\mathbb{R}$ a convex and subdifferentiable function. Denoting $\omega_{\theta}(\cdot)=\theta\omega\left(\frac{\cdot}{\theta}\right)$ for $\theta>0$ and $g_{\theta}=g\hspace{0.1cm}\square\hspace{0.1cm}\omega_{\theta}$. If we assume that $$D[g,\omega^*]=\sup_{x\in\R^d} \inf_{d\in \partial g(x)}\omega^*(d)<\infty$$ (where $\omega^*$ is the Fenchel conjugate of $\omega$), then: \begin{enumerate}
     \item $g(x)-D[g,\omega^*]\theta\leq g_{\theta}(x)\leq g(x)+\omega(0)\theta.$
     \item $g_{\theta}\in C_{\frac{1}{\sigma \theta}}^{1,1}(\mathbb{R}^d).$
 \end{enumerate}
 
  \end{proposition}
 \textbf{Note:} The Moreau envelope is a particular case of the previous Proposition with $\omega(x)=\frac{1}{2}\Vert x\Vert^2$, in particular Propositions \ref{nuevo}, \ref{nuevo1} and Corollary \ref{nuevocor} are still true if we use a strongly convex $\omega$.\\
 
 For the regularization $f\hspace{0.1cm}\square\hspace{0.1cm} \omega_{\theta}$, Proposition \ref{prim} stills true, the same thing happens for Proposition \ref{sc}, i.e., if $f\in{\Gamma_{c}}$ and $\omega\in\Gamma_{\lambda}$, then $f\hspace{0.1cm}\square\hspace{0.1cm} \omega_{\theta}\in \Gamma_{\frac{\lambda c}{\lambda+c\theta}}$, finally Proposition \ref{des} is also true for this regularization. 
\newpage
\section{Discrete setting}
Consider the Euler-Maruyama discretization of \eqref{CSGD} with stepsize $h$: \begin{equation}\label{discrete}
    x_{k+1}=x_k-h\nabla f(x_k)+\sigma(k,x_k)\triangle W_k,
\end{equation}
where $\triangle W_k=W((k+1)h)-W(kh)$.\\

And the piecewise linear continuous version \begin{equation}
    \tilde{X}(t):=x_k-(t-kh)\nabla f(x_k)+\sigma(k,x_k)(W(t)-W(kh)), \text{for } t\in [kh,(k+1)h] .
\end{equation}

Or equivalently 
\begin{equation}
    \tilde{X}(t)=x_0-\int_0^t \nabla f(\hat{X}(s))ds+\int_0^t \sigma(s,\hat{X}(s)) dB(s).
\end{equation}
Where $\hat{X}(t)=x_k$ for $t\in [kh,(k+1)h)$, and its called piecewise constant continuous version.\\

Assume that for every $T>0$ there exists some $p>2$ and a constant $A=A(T)$ such that \begin{equation}\label{assumption}
    \mathbb{E}\left(\sup_{0\leq t\leq T} |\tilde{X}(t)|^p\right)\vee \mathbb{E}\left(\sup_{0\leq t\leq T} |X(t)|^p\right)\leq A,
\end{equation}
where $X$ is a solution of \eqref{CSGD}.
\begin{lemma}\label{bound}
 If $X$ is a stochastic process such that $\mathbb{E}(\Vert X(t)\Vert^2)\leq C.$ Then $$\mathbb{E}(\Vert\overline{X(t)}\Vert^2)\leq \mathbb{E}(\overline{\Vert X(t)\Vert}^2)\leq\mathbb{E}(\overline{\Vert X(t)\Vert^2})\leq C.$$
\end{lemma}
\begin{proof}
The first inequality is direct from the fact that $| \int g(t)dt|\leq \int|g(t)|dt$. The last inequality is direct from integrate both sides of the hypothesis from $0$ to $t$ and then divide by $t$ (and exchange the expectation with the integral using Fubini). The middle inequality comes directly from the Cauchy-Schwarz Inequality for integrals, indeed \begin{align*}
\mathbb{E}(\overline{\Vert X(t)\Vert}^2)
&=\mathbb{E}\left(\left[\frac{1}{t}\int_0^t \Vert X(s)\Vert\right]^2\right)\\
&=\frac{1}{t^2}\mathbb{E}\left(\left[\int_0^t \Vert X(s)\Vert\right]^2\right)\\
&\leq \frac{1}{t}\mathbb{E}\left(\int_0^t \Vert X(s)\Vert^2\right)=\mathbb{E}( \overline{\Vert X(t)\Vert^2}).
\end{align*}
\end{proof}
\begin{lemma}\label{useful}
Let $f\in C_\Lp^{1,1}(\R^d)$ a convex function and $X,Y$ two random variables, such that $\mathbb{E}(\Vert X\Vert^2)<\infty.$ Then there exists $C\geq 0$ $$\mathbb{E}(f(X)-f(Y))\leq C\sqrt{\mathbb{E}(\Vert X-Y\Vert^2)}.$$
\end{lemma}
\begin{proof}
Using the convexity and the Cauchy-Schwarz Inequality, we obtain
\begin{align*}
    \mathbb{E}(f(X)-f(Y))&\leq \mathbb{E}(\langle \nabla f(X), X-Y \rangle)\\
    &\leq \mathbb{E}(|\langle \nabla f(X), X-Y \rangle|)\leq \mathbb{E}(\Vert \nabla f(X)\Vert \Vert X-Y \Vert)\\
    &\leq \sqrt{\mathbb{E}(\Vert \nabla f(X)\Vert^2)}\sqrt{\mathbb{E} (\Vert X-Y \Vert^2)}.\\
\end{align*}
Using that $f$ has Gradient Lipschitz and using the inequality $|x+y|^2\leq 2|x|^2+2|y|^2$, we conclude that \begin{align*}
    \mathbb{E}(f(X)-f(Y))&\leq \sqrt{2(\Lp^2\mathbb{E}(\Vert X\Vert^2)+\Vert \nabla f(0)\Vert^2})\sqrt{\mathbb{E} (\Vert X-Y \Vert^2)}.
\end{align*}
\end{proof}
\begin{lemma}\label{lema0}
 Let $T>0$ and consider $\hat{X}$ the piecewise linear and piecewise constant continuous version of (\ref{discrete}) with stepsize $h$. Then, for $t\in [0,T]$ we have $$\mathbb{E}(f(\overline{\hat{X}(t)})-f(\overline{\tilde{X}(t)}))= \mathcal{O}(h^{1/2}).$$
\end{lemma}
\begin{proof}
First, notice that $$\mathbb{E}\left(\sup_{t\in [0,T]}\Vert \hat{X}(t)\Vert^2\right)\leq \mathbb{E}\left(\sup_{t\in [0,T]}\Vert \tilde{X}(t)\Vert^2\right)\leq A^{2/p}.$$ By Lemma \ref{bound}, then $\mathbb{E}(\Vert \overline{\hat{X}(t)}\Vert^2)\leq A^{2/p}$ for every $t\in [0,T]$. Let $t\in [0,T]$, using Lemma \ref{useful} with $X=\overline{\hat{X}(t)}$, $Y=\overline{\tilde{X}(t)}$ we deduce that:
$$\mathbb{E}(f(\overline{\hat{X}(t)})-f(\overline{\tilde{X}(t)}))\leq C\sqrt{\mathbb{E}(\Vert \overline{\hat{X}(t)-\tilde{X}(t)}\Vert^2)}.$$
Finally, Lemma \ref{lemawe} says that $\mathbb{E}\left(\sup_{t\in [0,T]}\Vert \hat{X}(t)-\tilde{X}(t)\Vert^2\right)=\mathcal{O}(h)$. Using Lemma \ref{bound} again, we conclude that
$$\mathbb{E}(f(\overline{\hat{X}(t)})-f(\overline{\tilde{X}(t)}))=\mathcal{O}(h^{1/2}).$$
\end{proof}
\begin{corollary}\label{lema1}
 Let $T>0$ and consider $(x_k)_{k\in\N}$ generated by (\ref{discrete}) with stepsize $h$ and $kh\leq T$. Let $\tilde{X}$ its piecewise linear continuous version, then 
   $$\mathbb{E}(f(\overline{x_k})-f(\overline{\tilde{X}}(kh)))=\mathcal{O}(h^{1/2}).$$ 
\end{corollary}
%\begin{proof}
%First, we note that \begin{align*}
%    f(\tilde{X}(kh))= f\left(\frac{1}{kh}\int_0^{kh} \tilde{X}(s)ds\right)&=f\left(\frac{1}{kh}\sum_{i=0}^{k-1}\int_{ih}^{(i+1)h} x_i-(s-ih)\nabla f(x_i) +\sigma(i,x_i)(W(s)-W(ih)) ds\right)\\
%    &=f(\overline{x_k}-\frac{h}{2}\overline{\nabla f(x_k)}+\overline{\sigma(k,x_k)Z_k}).
%\end{align*}
%Where $(Z_i)_{i=0}^{k-1}$ is an i.i.d sequence of random vectors in $\R^d$ with distribution $\mathcal{N}(0,\frac{h}{3}I)$. By convexity of $f$ we can bound the term of interest:

%\begin{align*}
%\mathbb{E}(f(\overline{x_k})-f(\overline{\tilde{X}}(kh)))&\leq \mathbb{E}\left(-\langle \nabla f(\overline{x_k}), -\frac{h}{2}\overline{\nabla f(x_k)}+\overline{\sigma(k,x_k)Z_k}\rangle\right)\\
%&=\mathbb{E}\left(-\langle \nabla f(\overline{x_k}), -\frac{h}{2}\overline{\nabla f(x_k)}\rangle\right)+\mathbb{E}\left( -\langle \nabla f(\overline{x_k}),\overline{\sigma(k,x_k)Z_k}, \rangle\right) \\
%\end{align*}
%The first term is bounded in the following way:
%\begin{align*}
%\mathbb{E}\left(-\langle \nabla f(\overline{x_k}), -\frac{h}{2}\overline{\nabla f(x_k)}\rangle\right) & \leq \frac{h}{2}\mathbb{E}(\Vert \nabla f(\overline{x_k})\Vert\Vert\overline{\nabla f(x_k)}\Vert)\leq \frac{h}{2}\mathbb{E}\left( (L\Vert\overline{x_k}\Vert+\Vert\nabla f(0)\Vert)(L\overline{\Vert x_k\Vert}+\Vert \nabla f(0)\Vert) \right)\\
%&\leq \frac{h}{2}\mathbb{E}\left((L\overline{\Vert x_k\Vert}+\Vert\nabla f(0)\Vert)^2\right)=\frac{h}{2}\mathbb{E}\left( \Lp^2\overline{\Vert x_k\Vert}^2 +2\Vert \nabla f(0)\Vert \overline{\Vert x_k\Vert}+\Vert\nabla f(0)\Vert^2\right)\\
% \end{align*}
%By Cauchy Schwarz, we have that $\overline{\Vert x_k\Vert}^2\leq \overline{\Vert x_k\Vert^2}$. Then, using the assumption of (\ref{assumption}) along with the Jensen Inequality for concave functions, we obtain that
% $$\mathbb{E}\left(-\langle \nabla f(\overline{x_k}), -\frac{h}{2}\overline{\nabla f(x_k)}\rangle\right)\leq \frac{h}{2}[\Lp^2A^{2/p}+2L\Vert \nabla f(0)\Vert A^{1/p}+\Vert \nabla f(0)\Vert^2]=\mathcal{O}(h).$$
% The second term is bounded as follows:
% \begin{align*}
%     \mathbb{E}\left( -\langle \nabla f(\overline{x_k}),\overline{\sigma(k,x_k)Z_k} \rangle\right)&\leq \mathbb{E}\left(\Vert\nabla f(\overline{x_k})\Vert\Vert\overline{\sigma(k,x_k)Z_k}\Vert\right)\leq \sqrt{\mathbb{E}\left(\Vert \nabla f(\overline{x_k})\Vert^2\right)}\sqrt{\mathbb{E}\left(\Vert \overline{\sigma(k,x_k)Z_k}\Vert^2\right)}\\
%     &\leq \sqrt{2(\Lp^2\mathbb{E}(\Vert \overline{x_k}\Vert^2)+\Vert\nabla f(0)\Vert^2)}\sqrt{\mathbb{E}\left(\overline{\Vert \sigma(k,x_k)Z_k\Vert^2}\right)}\\
%     &\leq \sqrt{2(\Lp^2A^{2/p}+\Vert \nabla f(0)\Vert^2)}\sqrt{\sigma_*^2 d\overline{\mathbb{E}(\Vert Z_k\Vert^2)}}\\
%     &=\sqrt{2(\Lp^2A^{2/p}+\Vert \nabla f(0)\Vert^2)}\sqrt{\sigma_*^2 d\frac{dh}{3}}=\mathcal{O}(h^{1/2})
% \end{align*}
% And the conclusion is direct.
%\end{proof}
\begin{proof}
Note that $\overline{x_k}=\overline{\hat{X}(kh)}$. Thus, is direct from Lemma \ref{lema0} replacing $t=kh$.
\end{proof}
\begin{lemma}\label{lema2}
 Let $T>0$ and consider $(x_k)_{k\in\N}$ generated by (\ref{discrete}) with stepsize $h$. Let $\tilde{X}$ its piecewise linear continuous version and $t\in [0,T]$, then $$\mathbb{E}(f(\overline{\tilde{X}}(t))-f(\overline{X}(t)))= \mathcal{O}(h^{1/2})$$
\end{lemma}
%\begin{proof}
% Let $e(t)=\mathbb{E}\left( \overline{\Vert\tilde{X}(t)-X(t)\Vert}^2\right)$. Using convexity of $f$ and Cauchy Schwarz Inequality twice, we obtain:
% \begin{align*}
%         \mathbb{E}(f(\overline{\tilde{X}}(kh))-f(\overline{X}(kh)))&\leq \mathbb{E}\left(\langle \nabla f(\overline{\tilde{X}}(kh)),\overline{\tilde{X}}(kh)-\overline{X}(kh) \rangle\right)\leq \mathbb{E}\left(\Vert \nabla f(\overline{\tilde{X}}(kh))\Vert\Vert \overline{\tilde{X}}(kh)-\overline{X}(kh) \Vert\right)  \\
%         &\leq \mathbb{E}(\Vert\nabla f(\overline{\tilde{X}}(kh))\Vert \Vert\overline{\tilde{X}(kh)-X(kh)}\Vert)\leq \mathbb{E}(\Vert\nabla f(\overline{\tilde{X}}(kh))\Vert \overline{\Vert\tilde{X}(kh)-X(kh)\Vert}) \\%+\frac{L}{2}\mathbb{E}( \overline{\Vert\tilde{X}(kh)-X(kh)\Vert}^2)
%         &\leq \sqrt{\mathbb{E}\left(\Vert\nabla f\left(\overline{\tilde{X}}(kh)\right)\Vert^2\right)}\sqrt{e(kh)} \\%+\frac{L}{2}e(kh).
%         &\leq \sqrt{2(\Lp^2\mathbb{E}(\Vert \overline{\tilde{X}}(kh)\Vert^2)+\Vert\nabla f(0)\Vert^2)}\sqrt{e(kh)}\leq \sqrt{2(\Lp^2A^{2/p}+\Vert\nabla f(0)\Vert^2)}\sqrt{e(kh)}
%         \end{align*}
%        Where we have used the assumption of (\ref{assumption}) in the last inequality. By Minkowski Inequality, we can bound $$e(kh)\leq \frac{1}{k^2h^2} \left(\int_0^{kh} \mathbb{E}(\Vert \tilde{X}(s)-X(s) \Vert^2)^{1/2}ds\right)^2.$$
%         By \cite[Theorem 7.3]{gig} (see Lemma \ref{lemawe}), we have that $\mathbb{E}(\sup_{0\leq s\leq T}\Vert \tilde{X}(s)-X(s)\Vert^2)=\mathcal{O}(h)$.
%         This implies $e(kh)=\mathcal{O}(h)$. Then $$\mathbb{E}(f(\overline{\tilde{X}}(kh))-f(\overline{X}(kh)))=\mathcal{O}(h^{1/2}).$$
%\end{proof}
\begin{proof}
By hypothesis, $\mathbb{E}(\Vert \tilde{X}(t)\Vert^2)\leq A^{2/p}$ for every $t\in [0,T]$, then by Lemma \ref{bound}, $\mathbb{E}(\Vert \overline{\tilde{X}(t)}\Vert^2)\leq A^{2/p}$ for every $t\in [0,T]$. Using Lemma \ref{useful}, we obtain \begin{align*}
    \mathbb{E}(f(\overline{\tilde{X}}(t))-f(\overline{X}(t)))&\leq C\sqrt{\mathbb{E}(\Vert\overline{\hat{X}(t)-X(t)}\Vert^2)}.
\end{align*} 
By \cite[Theorem 7.3]{gig} (see Theorem \ref{aproxx}), we have that $\mathbb{E}\left(\sup_{0\leq t\leq T}\Vert \tilde{X}(t)-X(t)\Vert^2\right)=\mathcal{O}(h).$ Using Lemma \ref{bound}, we conclude that $$\mathbb{E}(f(\overline{\tilde{X}}(t))-f(\overline{X}(t)))=\mathcal{O}(h^{1/2}).$$
\end{proof}

\begin{proposition}\label{final}
 Let $T>0$ and consider $\hat{X}$ the piecewise constant version of (\ref{discrete}) with stepsize $h$,then for every $t\in [0,T]$ \begin{equation}
     \mathbb{E}\left[f\left(\overline{\hat{X}(t)}\right)\right]-min(f)=\mathcal{O}\left(\frac{1}{t}\right)+\mathcal{O}(h^{1/2})+\frac{\sigma_*^2 d}{2}.
 \end{equation}
\end{proposition}

\begin{proof} 
 $$\mathbb{E}(f(\overline{\hat{X}(t)}))-min(f)=\underbrace{\mathbb{E}(f(\overline{\tilde{X}(t)})-f(\overline{\tilde{X}}(t)))}_{(1)}+\underbrace{\mathbb{E}(f(\overline{\tilde{X}}(t))-f(\overline{X}(t)))}_{(2)}+\underbrace{\mathbb{E}(f(\overline{X}(t)))-min(f)}_{(3)}.$$
 
The term (1) is $\mathcal{O}(h^{1/2})$ by Corollary \ref{lema1}, the term (2) is $\mathcal{O}(h^{1/2})$ by Lemma \ref{lema2} and the term (3) can be bounded using the first item of Theorem \ref{importante0}.
Putting everything together, we obtain that there exists $C_1=C_1(T)$ such that $$\mathbb{E}(f(\overline{\tilde{X}(t)}))-min(f)\leq  C_1h^{1/2}+\frac{d^2(x_0,S)}{2t}+\frac{\sigma_*^2 d}{2}.$$
\end{proof}
\textbf{Note:} Notice that the first term of the upper bound is the discretization error, followed by the upper bound of the continuous case.
\begin{corollary}
 Let $T>0$ and consider $(x_k)_{k\in\N}$ generated by (\ref{discrete}) with stepsize $h$ and $kh\leq T$,then \begin{equation}
     \mathbb{E}(f(\overline{x_k}))-min(f)=\mathcal{O}(h^{1/2})+\mathcal{O}\left(\frac{1}{kh}\right)+\frac{\sigma_*^2 d}{2}.
 \end{equation}
\end{corollary}
\begin{proof}
Note that $\overline{x_k}=\overline{\hat{X}(kh)}$. Thus, is direct from Proposition \ref{final} replacing $t=kh$.
\end{proof}

\begin{proposition}
 Let $f\in C_\Lp^{1,1}(\R^d)\cap \Gamma_{\mu}(\R^d)$, $x^*$ a minimizer of $f$, $T>0$ and consider $\hat{X}$ the piecewise constant version of (\ref{discrete}) with stepsize $h$,then for every $t\in [0,T]$ there exists $C_2=C_2(T)$ such that \begin{equation}
     \mathbb{E}\left[\frac{\Vert\hat{X}(t)-x^*\Vert^2}{2}\right]\leq C_2h+ 2\Vert X_0-x^*\Vert^2e^{-\mu t}+\frac{2\sigma_*^2 d}{\mu}.
 \end{equation}
\end{proposition}

\begin{proof}
Let $t\in [0,T]$, then \begin{align*}
    \mathbb{E}\left[\frac{\Vert \hat{X}(t)-x^*\Vert^2}{2}\right]\leq \mathbb{E}\left[\Vert \hat{X}(t)-\tilde{X}(t)\Vert^2\right] +
    2\mathbb{E}\left[\Vert \tilde{X}(t)-X(t)\Vert^2\right] +
    4\mathbb{E}\left[\frac{\Vert X(t)-x^*\Vert^2}{2}\right] .
\end{align*}
By Lemma \ref{lemawe} and Theorem \ref{aproxx}, we have that the first two terms are $\mathcal{O}(h)$, for the last term, we use Theorem \ref{importante0} and we conclude.
\end{proof}

%\begin{proposition}
%  Let $f\in C_\Lp^{1,1}(\R^d)\cap Ł^{q}(\R^d)$, ($q\geq\frac{1}{2}$) $x^*$ a minimizer of $f$, $T>0$ and consider $\hat{X}$ the piecewise constant version of (\ref{discrete}) with stepsize $h$, for every $t\in [0,T]$ there exists $C_2=C_2(T)$, such that:
%  \begin{enumerate}
%      \item If $q=\frac{1}{2}$, then there exists $\mu>0$ such that
%      \begin{equation}
%     \mathbb{E}\left[\frac{d(\hat{X}(t),S)^2}{2}\right]\leq C_2h+ 2d(X_0,S)^2e^{-\frac{\mu_r^2}{2} t}+\frac{8\sigma_*^2 d}{\mu_r^2}.
% \end{equation}
% \item If $q>\frac{1}{2}$, then there exists $\tilde{\mu}>0$ such that
% \begin{equation}
%     \mathbb{E}\left[\frac{d(\hat{X}(t),S)^2}{2}\right]\leq C_2h+ 2\left(d(X_0,S)^{-\frac{2q-1}{1-q}}+\tilde{\mu}(p-2)t\right)^{-\frac{2(1-q)}{2q-1}}+2\left(\frac{\sigma_*^2 d}{\tilde{\mu}}\right)^{2(1-q)}
% \end{equation}
%  \end{enumerate}
  
%\end{proposition}
%\begin{proof}
%Let $t\in [0,T]$, then \begin{align*}
%    \mathbb{E}\left[\frac{d(\hat{X}(t),S)^2}{2}\right]\leq\mathbb{E}\left[\Vert\hat{X}(t)-\tilde{X}(t))\Vert^2\right]+2\mathbb{E}\left[\Vert\tilde{X}(t)-X(t))\Vert^2\right]+4\mathbb{E}\left[\frac{d(X(t),S)^2}{2}\right].
%\end{align*}
%By Lemma \ref{lemawe} and Theorem \ref{aproxx}, we have that the first two terms are $\mathcal{O}(h)$, for the last term, we use the Theorem \ref{importante} and we conclude both cases.
%\end{proof}


%\textbf{Note:} The purpose of the previous Proposition was to obtain a complexity rate of the discrete setting, nevertheless the dependance of $C_1$ with $T$ is exponential and we have results for $kh\leq T$, this fact makes the analysis worthless due to the first term is not bounded in a sharp way. (?)

